Algorithmic recourse under imperfect causal knowledge: a probabilistic approach

Recent work has discussed the limitations of counterfactual explanations to recommend actions for algorithmic recourse, and argued for the need of taking causal relationships between features into consideration. Unfortunately, in practice, the true underlying structural causal model is generally unknown. In this work, we first show that it is impossible to guarantee recourse without access to the true structural equations. To address this limitation, we propose two probabilistic approaches to select optimal actions that achieve recourse with high probability given limited causal knowledge (e.g., only the causal graph). The first captures uncertainty over structural equations under additive Gaussian noise, and uses Bayesian model averaging to estimate the counterfactual distribution. The second removes any assumptions on the structural equations by instead computing the average effect of recourse actions on individuals similar to the person who seeks recourse, leading to a novel subpopulation-based interventional notion of recourse. We then derive a gradient-based procedure for selecting optimal recourse actions, and empirically show that the proposed approaches lead to more reliable recommendations under imperfect causal knowledge than non-probabilistic baselines.

==> sec/7_results.tex <==
\paragraph{Plots that would be nice to include here:}
\begin{itemize}
    \item plots of validity (and maybe also cost) (y-axis) of  different models (or a relevant subset thereof) evaluated on the same SCM but for different values of the linearity/additivity/Gaussianity parameters $a,b,c$ (x-axis) $\implies $ this shows the robustness of the different approaches to assumptions about the underlying SCM
    \item plots of cost vs. validity for a single approach evaluated on the same SCM but for different values of $\lambda_{\LCB}$ (somewhat akin to a Pareto front) $\implies$ this shows how, for the probabilistic approaches, $\lambda_{\LCB}$ can be used to trade-off higher validity at the expense of higher cost (generally speaking)
    \item (optionally, if we have time:) plots about how the number of Monte Carlo samples, learning rate, and other aspect about the optimisation procedure influence each other and the objective function
\end{itemize}
